A Sorted Datalog Hammer for Supervisor Verification Conditions Modulo Simple Linear Arithmetic

In a previous paper, we have shown that clause sets belonging to the Horn Bernays-Sch\"onfinkel fragment over simple linear real arithmetic (HBS(SLR)) can be translated into HBS clause sets over a finite set of first-order constants. The translation preserves validity and satisfiability and it is still applicable if we extend our input with positive universally or existentially quantified verification conditions (conjectures). We call this translation a Datalog hammer. The combination of its implementation in SPASS-SPL with the Datalog reasoner VLog establishes an effective way of deciding verification conditions in the Horn fragment. We verify supervisor code for two examples: a lane change assistant in a car and an electronic control unit of a supercharged combustion engine. In this paper, we improve our Datalog hammer in several ways: we generalize it to mixed real-integer arithmetic and finite first-order sorts; we extend the class of acceptable inequalities beyond variable bounds and positively grounded inequalities; and we significantly reduce the size of the hammer output by a soft typing discipline. We call the result the sorted Datalog hammer. It not only allows us to handle more complex supervisor code and to model already considered supervisor code more concisely, but it also improves our performance on real world benchmark examples. Finally, we replace the before file-based interface between SPASS-SPL and VLog by a close coupling resulting in a single executable binary.

==> implementation.tex <==
\section{Implementation as a Decision Procedure} \label{sec:implementation}

We have implemented the Datalog hammer into our \BS(\LRA) system SPASS-SPL and combined it with the Datalog reasoner Rulewerk.
The resulting toolchain is the first implementation of a decision procedure for \HBS(\SB) with positive conjectures.

\subsubsection{SPASS-SPL} 
is a new system for $BS(\LRA)$ based on some core libraries of our first-order
theorem prover SPASS~\cite{WeidenbachEtAlSpass2009} and including our CDCL(LA) solver SPASS-SATT~\cite{BrombergerEtAl19} for mixed linear arithmetic.
Eventually, SPASS-SPL will include a family of reasoning techniques for $BS(\LRA)$ including SCL(T)~\cite{BrombergerFW21},
hierarchic superposition~\cite{BachmairGanzingerEtAl94,BaumgartnerWaldmann19} and hammers to various logics.
Currently, it comprises the Datalog hammer described in this paper and hierarchic UR-resolution~\cite{McCharenOverbeekEtAl76} (Unit Resulting resolution)
which is complete for $\HBS(\LRA)$.
The Datalog hammer can produce the clause format used in the Datalog system \emph{Rulewerk} (described below), but also the SPASS first-order logic clause format that can then
be translated into the first-order TPTP library~\cite{Sutcliffe17} clause format.
Moreover, it can be used as a translator from our own input language into the SMT-LIB 2.6 language and the CHC competition format.

Note that our implementation of the Datalog hammer is not fully mature. 
It cannot handle positively grounded theory atoms beyond simple bounds, unless they are variable comparisons (i.e., $x \LAOP y$ with $\LAOP \in \{\leq, <, \neq, =, >, \geq\}$) or defined separately in the input file as so called theory patterns.
Moreover, positive universal conjectures have to be flattened by hand until they have the form $\Lambda \parallel P(\bar{x})$.
On the other hand, we already added some minor optimizations, e.g., we can exploit the theory atoms $\Lambda$ in a universal conjecture $\Lambda \parallel P(\bar{x})$ so the hammered conjecture only contains those groundings for $P(\bar{x})$ that satisfy $\Lambda$.

\subsubsection{Rulewerk}
(formerly \emph{VLog4j}) is a rule reasoning toolkit that consists of a Java API and an
interactive shell \cite{Rulewerk2019}. Its current main reasoning back-end is the rule engine \emph{Vlog} \cite{UJK:VLog2016}, which supports
Datalog and its extensions with stratified negation and existential quantifiers, respectively.
VLog is an in-memory reasoner that is optimized for efficient use of resources, and has been
shown to deliver highly competitive performance in benchmarks \cite{UKJDC18:VLogSystemDescription}.

We have not specifically optimized VLog or Rulewerk for this work, but we have tried to select Datalog
encodings that exploit the capabilities of these tools. The most notable impact was observed for the
encoding of universal conjectures. A direct encoding of (grounded) universal claims in Datalog
leads to rules with many (hundreds of thousands in our experiments) of ground atoms as their precondition. Datalog reasoners (not just
VLog) are not optimized for such large rules, but for large numbers of facts.
An alternative encoding in plain Datalog would therefore specify the expected atoms as facts and
use some mechanism to iterate over all of them to check for goal. To accomplish this iteration, the facts
that require checking can be endowed with an additional identifier (given as a parameter), and an auxiliary
binary successor relation can be used to specify the iteration order over the facts. This approach requires only
few rules, but the number of rule applications is proportional to the number of expected facts.

In Rulewerk/VLog, we can encode this in a simpler way using negation.
Universal conjectures require us to evaluate ground queries of
the form $\textit{entailed}(\bar{c}_1)\wedge\ldots\wedge\textit{entailed}(\bar{c}_\ell)$. 
If we add facts $\textit{expected}(\bar{c}_i)$ for the constant vectors $\bar{c}_1,\ldots,\bar{c}_\ell$,
we can equivalently use a smaller (first-order) query 
$\forall\bar{x}.(\textit{expected}(\bar{x})\to\textit{entailed}(\bar{x}))$, which 
in turn can be written as
$\neg\big(\exists\bar{x}.(\textit{expected}(\bar{x})\wedge\neg\textit{entailed}(\bar{x}))\big)$.
This can be expressed in Datalog with negation, where \textit{Goal} encodes that the query matches:
\begin{align}
\textit{expected}(\bar{x})\wedge\neg\textit{entailed}(\bar{x}) &\to \textit{missing} \label{rule_exp_missing}\\
\neg\textit{missing} &\to \textit{Goal} \label{rule_missing_goal}
\end{align}
This use of negation is \emph{stratified}, i.e., not entwined with recursion \cite{Alice}.
Note that stratified negation is a form of non-monotonic negation, so we can no longer read such rules as first-order
formulae over which we compute entailments. Nevertheless, implementation is simple and stratified negation is a widely
supported feature in Datalog engines, including Rulewerk.
The encoding is particularly efficient since each of the rules \eqref{rule_exp_missing} and \eqref{rule_missing_goal} is evaluated only once.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

